Multi-Label Gold Asymmetric Loss Correction with Single-Label Regulators

Multi-label learning is an emerging extension of the multi-class classification where an image contains multiple labels. Not only acquiring a clean and fully labeled dataset in multi-label learning is extremely expensive, but also many of the actual labels are corrupted or missing due to the automated or non-expert annotation techniques. Noisy label data decrease the prediction performance drastically. In this paper, we propose a novel Gold Asymmetric Loss Correction with Single-Label Regulators (GALC-SLR) that operates robust against noisy labels. GALC-SLR estimates the noise confusion matrix using single-label samples, then constructs an asymmetric loss correction via estimated confusion matrix to avoid overfitting to the noisy labels. Empirical results show that our method outperforms the state-of-the-art original asymmetric loss multi-label classifier under all corruption levels, showing mean average precision improvement up to 28.67% on a real world dataset of MS-COCO, yielding a better generalization of the unseen data and increased prediction performance.

==> algo_1.tex <==
\begin{algorithm}[tb]
\caption{GLC $\widehat{\boldsymbol{C}}$ estimation}\label{alg:glc_c_hat_estimation}
\begin{algorithmic}[1]
\State \textbf{Input:} \text{Untrusted data $\mathcal{S}$, silver classifier $f$}
\State $K = $ \text{number of possible labels}
\State \textcolor{lightgray}{\textit{/* Estimate single-label corruption matrix */}}
\State \text{Fill} $\widehat{\boldsymbol{C}} \in \mathbb{R} ^{K \times K}$ \text{with zeros}
\State \textcolor{lightgray}{\textit{/* For each label, calculate its corruption row by taking the mean silver softmax predictions over the untrusted samples */}}
\For{$k = 1,...,K$}
    \State $num\_examples = 0$
    \State \textcolor{lightgray}{\textit{/* For each single-label image of label k */}}
    \For{$(\boldsymbol{x}_{i}, \boldsymbol{y}_{i}) \in \mathcal{S}$ \text{such that} $\boldsymbol{y}_{ik} = 1$}
        \State $num\_examples += 1$
        \State \textcolor{lightgray}{\textit{/* Add silver softmax prediction to $k$th row */}}
        \State $\widehat{\boldsymbol{C}}_{k\bullet} += f_{soft}(x_{i})$
    \EndFor
    \State \textcolor{lightgray}{\textit{/* Divide row $k$ by the number of samples */}}
    \State $\widehat{\boldsymbol {C}}_{k\bullet} /= num\_examples$
\EndFor
\end{algorithmic}
\end{algorithm}

==> algo_ouput_correction.tex <==
\begin{algorithm}[tb]
\caption{GALC-SLR Output correction}\label{alg:galc-slr_output_correction}
\begin{algorithmic}[1]
\State \textbf{Input:} \text{Multi-label corruption matrix $\widehat{\boldsymbol{C}}$}
\State \textbf{Input:} \text{Untrained classifier $g$}
\State \textbf{Input:} \text{Data sample $(\boldsymbol{x}_{i}, \boldsymbol{y}_{i})$}
\State $K = $ \text{number of possible labels}
\State \textcolor{lightgray}{\textit{/* Calculate overall Correction by taking the mean of correction rows $\widehat{\boldsymbol{C}}^{T}$ over all target labels */}}
\State \text{Fill} $Corr \in \mathbb{R} ^{K}$ \text{with zeros}
\State $num\_labels = 0$
\State \textcolor{lightgray}{\textit{/* Initial sigmoid output of our untrained classifier */}}
\State $\widehat s = g_{sig}(\boldsymbol{x}_{i})$
\State \textcolor{lightgray}{\textit{/* For each label that occurs in the image */}}
\For{$k = 1,...,K$ \text{such that} $\boldsymbol{y}_{ik} = 1$}
    \State $num\_labels += 1$
    \State \textcolor{lightgray}{\textit{/* Add correction row of $\widehat C$ transpose */}}
    \State $Corr += \widehat{\boldsymbol{C}}^{T}_{k\bullet}$
\EndFor
\State \textcolor{lightgray}{\textit{/* Divide by the number of labels */}}
\State $Corr /= num\_labels$
\State \textcolor{lightgray}{\textit{/* Define the corrected output */}}
\State $s = Corr * \widehat s$
\end{algorithmic}
\end{algorithm}

==> relatedwork.tex <==
Recent literature has shown increased interest towards robustness against noisy labels in training, much more in single-label classification than in multi-label learning. We first investigate a few robust solutions in multi-label classification, followed by an analysis in a single-label context. Lastly, we describe the overall mechanism of GLC and outline its main strengths and weaknesses.

\subsection{Single-label Classification}
Many researchers have been tackling the problem of noisy labels in single-label classification. \citep{surveydnnnoisylabels} is providing a comprehensive evaluation of 57 state-of-the-art robust DNNs. For a very detailed analysis we strongly recommend the reader to check the paper from which we briefly mention a few of the robust solutions. The paper clearly distinguishes between five categories of robust DNNs. Some classifiers such as C-model \citep{cmodel}, Contrastive-Additive Noise Network \citep{cann} and Robust Generative Classifier (RoG) \citep{rog} have been shaped to have a Robust Architecture by “adding a noise adaptation layer at the top of the softmax layer”. Another solution is to use the well-known regularization techniques such as data augmentation \citep{dataaug}, weight decay \citep{weighdecay}, dropout \citep{dropout} and batch normalization \citep{batchnorm}. These methods perform well on low to moderate noise, but fail on datasets with higher noise \citep{regulestimation}. Other solutions use Sample Selection and have shown impressive results, most of them being robust even to heavy noise. A few popular examples are MentorNet \citep{mentornet}, Co-teaching \citep{coteaching} and Co-teaching+ \citep{coteaching+}.

\subsection{Multi-label Classification}
In multi-label learning, little attention has been given to the consequences of label noise. \citep{evaluatingmllclassifiersnoisylabels} is one of the few papers that treats the problem of noisy labels in a multi-label context.
The paper proposes a Context-Based Multi-Label Classifier (CbMLC) ``that effectively handles noisy labels when learning label dependencies''. Another solution is the Multivariate Probit Variational AutoEncoder (MPVAE)
~\citep{mpvae}, method that outperforms many other classifiers in multiple application domains and, furthermore, has been proven to remain robust under medium label noise. Even though robustness was not the main goal of MPVAE, the researchers have also analyzed this matter in their paper, acknowledging the importance of the impact of noisy labels.



\subsection{Gold Loss Correction - GLC}
The last category consists of classifiers with Loss Adjustment such as the Loss Correction Approach. These methods are actively modelling the noise distribution by estimating a label corruption matrix. The Gold Loss Correction (GLC) \citep{glc} is powerful method that achieves impressive results under both symmetric and asymmetric noise and also against very heavy noise. GLC assumes that a small subset of the samples can be trusted and uses this extra information in order to accurately estimate the true corruption matrix, such as the one in Figure \ref{fig:corruption_matrix}. We consider GLC to be a very effective and simple approach in the single-label setting. However, their method works when the data is completely separable, meaning that y is deterministic given x. This is not the case in multi-label learning and, furthermore, the label correlations and the class imbalance in the training data make this problem even more difficult.

\begin{figure}[t!]
\centering
\includegraphics[width=0.4\columnwidth]{figures/TRUE Corruption Matrix_soft.pdf}
\caption{Corruption matrix for 80 labels - 40\% noise}
\label{fig:corruption_matrix}
\end{figure}


==> table_results.tex <==
\begin{table}[t!]
\centering
\caption{Evaluation results of ASL and GALC-SLR on MS-COCO}
\label{tab:evaluation_results}
% \resizebox{0.9\columnwidth}{!}{%
\begin{tabular}{|c|c;{1pt/1pt}c;{1pt/1pt}c|c;{1pt/1pt}c;{1pt/1pt}c|} 
\hline
\rowcolor{gray!25} & \multicolumn{3}{c|}{ASL} & \multicolumn{3}{c|}{GALC-SLR} \\ 
\cline{2-7}
\rowcolor{gray!25} \multirow{-2}{*}{\textbf{Noise} } & \textbf{mAP} & \textbf{CF1} & \textbf{OF1} & \textbf{mAP} & \textbf{CF1} & \textbf{OF1}\\ 
\hline
\hline
\textit{0\%} & 74.91 & 71.38 & 75.55 & \textbf{75.08} & 70.82 & 75.09\\ 
\hline
\textit{10\%} & 69.55 & 68.01 & 73.07 & \textbf{74.54} & 70.55 & 74.85\\ 
\hline
\textit{20\%} & 64.71 & 64.03 & 69.96 & \textbf{73.77} & 69.66 & 74.25\\ 
\hline
\textit{30\%} & 58.89 & 58.52 & 65.30 & \textbf{71.85} & 68.27 & 73.41\\ 
\hline
\textit{40\%} & 52.18 & 52.24 & 59.58 & \textbf{69.94} & 66.45 & 72.28\\ 
\hline
\textit{50\%} & 45.24 & 45.42 & 52.78 & \textbf{68.31} & 64.68 & 71.33\\ 
\hline
\textit{60\%} & 36.81 & 37.44 & 43.29 & \textbf{65.48} & 61.73 & 69.42\\ 
\hline
\end{tabular}
% }
\end{table}
